Piecewise Flat Gravity in 3+1 dimensions

We study a model for gravity in 3+1 dimensions, inspired in general relativity in 2+1 dimensions. In contrast regular general relativity in 3+1 dimensions, the model postulates that space in absence of matter is flat. The requirement that the Einstein equation still holds for the complete spacetime, implies that matter may only appear as conical defects of co-dimension 2, which may be interpreted as straight cosmic strings moving at a constant velocity. The study of collisions of these defects reveals that the dynamics of the model is incomplete. Certain highly energetic collisions of almost parallel defects suggest that no dynamic completion may exist that is fully compatible with the principles on which the model was based. We also study the phase space of the model in the continuum limit. We find that even though does not contain gravitational waves at the fundamental level, they do appear as an emergent feature in the continuum limit.

==> meta/frontpage.tex <==
% !TeX root =../ThesisMvdM.tex

\thispagestyle{empty}
\phantom{}
\vspace{2.0cm}

\begin{center}
{\fontshape{sc}
\fontsize{32}{32}\selectfont
Piecewise flat gravity\\[9pt]
\fontsize{24}{24}\selectfont
in 3+1 dimensions}
\end{center}

\newpage
\thispagestyle{empty}
\phantom{}
\vfill
\noindent van de Meent, Maarten\\[3mm]
\noindent Piecewise flat gravity in 3+1 dimensions\\
\noindent PhD thesis\\
\noindent Institute for Theoretical Physics\\
\noindent Utrecht University\\
\noindent ISBN: 978-90-393-5697-5\\
\noindent printed by Gildeprint Drukkerijen te Enschede

